Constant Mean Curvature n-noids with Platonic Symmetries

Constant Mean Curvature n-noids with Platonic Symmetries

==> figure1.tex <==
\begin{figure}[ht]
  \centering
  \includegraphics[scale=0.115]{images/noid3.eps}
  \includegraphics[scale=0.1]{images/starnoid4.eps}
  \includegraphics[scale=0.115]{images/starnoid5.eps}
%\end{figure}
%\begin{figure}[ht]
  \centering
  \includegraphics[scale=0.115]{images/starnoid6.eps}
  \includegraphics[scale=0.115]{images/starnoid7.eps}
  \includegraphics[scale=0.115]{images/starnoid8.eps}
\caption{
CMC surfaces in $\bbR^3$ with prismatic symmetry.}
\end{figure}


==> figure2.tex <==
\begin{figure}[ht]
  \centering
%  \includegraphics[scale=0.115]{images/noid3.eps}
  \includegraphics[scale=0.15]{images/podnoid4.eps}
%  \includegraphics[scale=0.115]{images/podnoid5.eps}
%\end{figure}
%\begin{figure}[ht]
  \centering
  \includegraphics[scale=0.15]{images/podnoid6.eps}
%  \includegraphics[scale=0.115]{images/podnoid7.eps}
%  \includegraphics[scale=0.3]{images/podnoid8.eps}
\caption{CMC surfaces in $\bbR^3$.
The tetranoid (right) has full tetrahedral symmetry.
The example on the left has pyramidal symmetry.}
\end{figure}


==> figure3.tex <==
\begin{figure}[ht]
  \centering
  \includegraphics[width=2.4in]{images/cube1.eps}
  \includegraphics[width=2.4in]{images/cube2.eps}
\caption{CMC surfaces in $\bbR^3$ with six ends and full octahedral symmetry.
These examples have the end behavior of unduloids (left)
and nodoids (right, cutaway view).}
\end{figure}


==> figure4.tex <==
\begin{figure}[ht]
  \centering
  \includegraphics[width=5in]{images/parallel.eps}
\caption{Cutaway view of a CMC surface in $\bbR^3$ with pyramidal symmetry
and four parallel ends. The unduloidal end to the right has weight
$1/2$ and the coaxial nodoidal end to the left has weight $-1/3$.
The two remaining unduloidal ends,
of which only one is visible, each has weight
$5/12$. The total of the weights, taking into account the end directions,
is $0$.}
\end{figure}


==> figure5.tex <==
\begin{figure}[ht]
  \centering
  \includegraphics[width=2.4in]{images/cyclic.eps}
  \includegraphics[width=2.4in]{images/dihedral.eps}
\caption{CMC $n$-noids with pyramidal and prismatic symmetries.
The pyramidal example (left) has unduloid and nodoid ends sharing
an axial line, plus four more equal-weight ends.
The prismatic example (right) has
equal-weight unduloid ends sharing an axial line,
plus six alternate unduloidal and nodoidal ends.}
\end{figure}


==> figure6.tex <==
\begin{figure}[ht]
  \centering
  \includegraphics[width=2.2in]{images/hexahedral.eps}
  \includegraphics[width=2.6in]{images/octahedron.eps}
\caption{CMC $n$-noids with octahedral symmetry,
with eight ends (left)
and six ends (right).}
\end{figure}


==> figure7.tex <==
\begin{figure}[ht]
  \centering
  \includegraphics[width=2.4in]{images/dodecahedral.eps}
  \includegraphics[width=2.4in]{images/icosahedral.eps}
  \caption{CMC $n$-noids with icosahedral symmetry,
with twelve ends (left)
and twenty ends (right).}
\end{figure}

